Deep Learning for Gamma-Ray Bursts: A data driven event framework for X/Gamma-Ray analysis in space telescopes

This thesis comprises the first three chapters dedicated to providing an overview of Gamma Ray-Bursts (GRBs), their properties, the instrumentation used to detect them, and Artificial Intelligence (AI) applications in the context of GRBs, including a literature review and future prospects. Considering both the current and the next generation of high X-ray monitors, such as Fermi-GBM and HERMES Pathfinder (an in-orbit demonstration of six 3U nano-satellites), the research question revolves around the detection of long and faint high-energy transients, potentially GRBs, that might have been missed by previous detection algorithms. To address this, two chapters introduce a new data-driven framework, DeepGRB. In Chapter 4, a Neural Network (NN) is described for background count rate estimation for X/gamma-ray detectors, providing a performance evaluation in different periods, including both solar maxima, solar minima periods, and one containing an ultra-long GRB. The application of eXplainable Artificial Intelligence (XAI) is performed for global and local feature importance analysis to better understand the behavior of the NN. Chapter 5 employs FOCuS-Poisson for anomaly detection in count rate observations and estimation from the NN. DeepGRB demonstrates its capability to process Fermi-GBM data, confirming cataloged events and identifying new ones, providing further analysis with estimates for localization, duration, and classification. The chapter concludes with an automated classification method using Machine Learning techniques that incorporates XAI for eventual bias identification.

==> tables/work_table.tex <==
% Table of works
\begin{longtable}{llp{4cm}p{2cm}p{4cm}r} %{p{2cm}p{2cm}p{2cm}p{2cm}p{3cm}r
\toprule
Study & Telescope & Method unsup. & Method sup. & Parameters & Clusters \\
\midrule
\endhead
%%% BATSE
\cite{hakkila1998ai} & BATSE & Conceptual clustering (CLASSIT) & Decision tree & T90, $P_{1024}$, $f_{23}$, $HR_{21}$, $H_{32}$, $HR_{43}$ & 2 \\
\cite{mukherjee1998three} & BATSE & Hierarchical agglomerative clustering, GMM & - & T50, T90, $P_{1024}$, $P_{256}$, $P_{64}$, $f$, $f_1$, $f_2$, $f_3$, $f_4$, $H_{3-21}$ & 3 \\ % F1-F4 in the 20-50 keV, 50-100 keV, 100-300 keV and > 300 keV
\cite{balastegui2005neural} & BATSE & SOM & - & T90, T50, $P_{1024}$, $P_{256}$, $P_{64}$, $f_1$, $f_2$, $f_3$, $f_4$, $HR_{32}$, $\frac{V}{V_{max}}$ & 3 \\
\cite{hakkila2000gamma} & BATSE & - & Decision tree & T90, T50, $P_{1024}$, $P_{256}$, $P_{64}$, $f_{23}$, $f_1$, $f_2$, $f_3$, $f_4$, $HR_{32}$, $HR_{21}$, $HR_{3-21}$, $HR_{43}$ & 2 \\
\cite{balastegui2001reclassification} & BATSE & PCA, Hierarchical clustering, Neural Network & - & T90, $P_{1024}$, $P_{256}$, $P_{64}$, $f_1$, $f_2$, $f_3$, $f_4$, & 3 \\
\cite{roiger2000unsupervised} & BATSE & Hierarchical clustering & Decision tree & T90, $f$, $HR_{3-21}$ & 4 \\
\cite{pereira2010combining} & BATSE & Self-organizing map, PCA & - & T90, T50, $f_1$, $f_2$, $f_3$, $f_4$, $HR_{3-21}$ & 5 \\
\cite{rajaniemi2002classifying} & BATSE & SOM & - & T90, $f_{23}$, $HR_{3-21}$ & 2 \\
\cite{hakkila2003sample} & BATSE & K-means, SOM, GMM & - & T90, $f$, $HR_{3-21}$ & 2 \\
\cite{chattopadhyay2007statistical} & BATSE & K-means, Dirichlet mixture & - & T50, T90, $f$, $P_{256}$, $HR_{3-21}$, $HR_{32}$ & 3 \\
\cite{goldstein2010new} & BATSE & Lognormal & - & $E_{peak}$, $f$ & 2 \\
\cite{modak2018clustering} & BATSE & K-means & - &  T90, T50, $P_{1024}$, $P_{256}$, $P_{64}$, $f_1$, $f_2$, $f_3$, $f_4$ & 3 \\
\cite{modak2021distinction} & BATSE & Fuzzy cluster (FANNY) & - &  T90, T50, $P_{1024}$, $P_{256}$, $P_{64}$, $f_1$, $f_2$, $f_3$, $f_4$, $HR_{32}$, $HR_{3-21}$ & 3 \\
%%% BeppoSAX
\cite{horvath2009classification} & BeppoSAX & Lognormal & - &  T90 & 3 \\
%%% Swift
\cite{horvath2008classification} & Swift & Lognormal & - & T90 & 3 \\
\cite{horvath2010detailed} & Swift & GMM & - & T90, $HR_{32}$ & 2 \\
\cite{lu2010new} & Swift & GMM & - & T90, $\epsilon$ & 2 \\

\cite{jespersen2020unambiguous} & Swift & T-sne & - & DTFT on lightcurve & 2 \\
\cite{misra2023evidence} & Swift & T-sne & - & DTFT on lightcurve & 5 \\
\cite{garcia2023identification} & Swift & T-sne & - & DTFT on lightcurve & 2 \\
\cite{berretta2022comprehension} & Swift & T-sne & - & DTFT on lightcurve & 2 \\
%%% Fermi
\cite{tarnopolski2015analysis} & Fermi & Lognormal & - &  T90 & 2 \\
\cite{tarnopolski2015distinguishing} & Fermi & - & SVM & T90, HE, MVTS & 2 \\
\cite{horvath2015classification} & Fermi & PCA, GMM & - &  T90, $f$, HR, $P_{256}$ & 3 \\
\cite{horvath2019multidimensional} & Fermi & PCA, GMM & - &  T90, T50, $f$, \textit{Fermi parameters} & 3 \\
\cite{zhang2022tight} & Fermi GBM & PCA, GMM, LDA & - &  T90, $f$, peak flux & 3 \\

%%% Multiple satellites
\cite{zhang2016classifying} & BATSE & GMM & - &  T90 ($f2$, $f3$, $HR_{23}$ used only for filter) & 2 \\
\cite{zhang2016classifying} & Swift & GMM & - &  T90 ($HR_{31}$ used only for filter) & 3 \\
\cite{zhang2016classifying} & Swift & GMM & - &  T90 adjusted for z ($HR_{31}$ used only for filter) & 2 \\
\cite{zhang2016classifying} & Fermi & GMM & - &  T90 ($f$, HR, flncCompIndex, lgflncCompEpeak used only for filter) & 2 \\

\cite{kulkarni2017classification} & BATSE & Lognormal & - &  T90 & 2 \\
\cite{kulkarni2017classification} & Fermi & Lognormal & - &  T90 & 2 \\
\cite{kulkarni2017classification} & BeppoSAX & Lognormal & - &  T90 & 2 \\
\cite{kulkarni2017classification} & Swift & Lognormal & - &  T90 & 3, 2 \\

\cite{tarnopolski2022graph} & RHESSI & Graph-based algorithms & - &  T90, $HR_{32}$ & 2 \\
\cite{tarnopolski2022graph} & Konus-Wind & Graph-based algorithms & - &  T90, $HR_{32}$ & 2 \\
\cite{tarnopolski2022graph} & BATSE & Graph-based algorithms & - &  T90, $HR_{32}$ & 2, 3 \\
\cite{tarnopolski2022graph} & Swift & Graph-based algorithms & - &  T90, $HR_{32}$ & 2 \\
\cite{tarnopolski2022graph} & Fermi & Graph-based algorithms & - &  T90, $HR_{32}$ & 2, 3 \\
\cite{tarnopolski2022graph} & Sazaku & Graph-based algorithms & - &  T90, $HR_{32}$ & 2 \\
\cite{desai2022two} & BATSE & Extended GMM (XDGMM) & - &  T90, $HR$ & 2 \\ % 50-100 keV and the 20-50 keV
\cite{desai2022two} & Fermi & Extended GMM (XDGMM) & - &  T90, $HR$ & 3 \\ %50-300 keV and 10-50 keV
\cite{salmon2022two} & Fermi & GMM & - &  T90, $HR$ & 2 \\ % 8–50 keV band to the 50–300 keV
\cite{salmon2022two} & Swift & GMM & - &  T90, $HR_{32}$ & 2 \\ % range 3 (50–100 keV) to energy range 2 (25–50 keV)
\cite{salmon2022twoGMM} & BATSE & t-SNE, PCA, GMM & - &  Wavelet transform on lightcurve & 2 \\
\cite{salmon2022twoGMM} & Fermi & t-SNE, PCA, GMM & - &  Wavelet transform on lightcurve & 2 \\
\cite{salmon2022twoGMM} & Swift & t-SNE, PCA, GMM & - &  Wavelet transform on lightcurve & 2 \\
\cite{luo2022identifying} & - & - & XGBoost &  T90, $f$, $HR$, z, spectral parameters, afterglow features, host galaxy features & 2 \\
\cite{steinhardt2023classification} & Swift & T-sne, UMAP & - & DTFT on lightcurve & 2 \\
\cite{steinhardt2023classification} & Fermi & T-sne, UMAP & - & DTFT on lightcurve & 2 \\
\cite{steinhardt2023classification} & BATSE & T-sne, UMAP & - & DTFT on lightcurve & 2 \\

\bottomrule \\
\caption{\label{tab:work_table} Summary table works. $P$ is the peak flux and the suffix specify the ms time binning, $f$ the fluence and the suffix specify the energy channels, $HR_{xy}$ the hardness ratio ($\frac{f_x}{f_y}$), $\frac{V}{V_{max}}$ is a measure of the maximum redshift, $\epsilon$ is based on the isotropic gamma-ray energy and the cosmic rest-frame spectral peak energy, MVTS is the minimum variability time-scales, HE the Hurst Exponents (a time series feature), z is the redshift when available. The \textit{Fermi parameters} are: lgPflux64 (64 ms peak flux), lgPflux256 (256 ms peak flux), lgPflux1024 (1024 ms peak flux), lgfluenceBATSE (fluence in the BATSE energy channels), lgPflux64BATSE (64 ms peak flux in the BATSE energy channels), lgPflux256BATSE, (256 ms peak flux in the BATSE energy channels), lgPflux1024BATSE(1024 ms peak flux in the BATSE energy channels), lgflncCompAmp (Compton amplitude from fluence spectral fit), lgflncCompEpeak (Compton Epeak from fluence spectral fit), flncCompIndex (Compton power law index from fluence spectral fit), lgpflxCompAmp (Compton amplitude from peak flux spectral fit), lgpPflxCompEpeak (Compton Epeak from peak flux spectral fit), and pflxCompIndex (Compton power law index from peak flux spectral fit). Notice that the channels depends on the instrument and sometimes it's different from work to work. DTFT stands for discrete-time Fourier transform.}
\end{longtable}
